HP-PnP-Flow: Hybrid Time Scheduling and Projection for Plug-and-Play Image Restoration via Flow Matching

Image restoration is a fundamental inverse problem that seeks to recover high-quality images from degraded observations. Plug-and-Play (PnP) methods provide a flexible framework for integrating pretrained denoisers into iterative reconstruction, whereas flow matching offers an efficient generative modeling approach based on continuous-time ODE dynamics. Very recently, Martin et al. (ICLR, 2025) developed a PnP-Flow method, which integrates the PnP framework with flow matching through a time-dependent denoiser constructed from a pretrained flow matching model. By incorporating a different time schedule and an additional pixel-space projection operator, this paper proposes a novel efficient PnP-Flow algorithm (HP-PnP-Flow) that enjoys rigorous convergence guarantees under mild assumptions, without imposing restrictive conditions on iterates required by the aforementioned work. Numerical experiments on CelebA and AFHQ-Cat demonstrate that the newly proposed HP-PnP-Flow algorithm significantly outperforms PnP-Flow on several restoration tasks such as denoising, deblurring, super-resolution, random inpainting, and box inpainting. Notably, our algorithm achieves comparable or better reconstruction quality with substantially fewer iterations, reducing the iteration count from $500$ to $100$ for deblurring and super-resolution on AFHQ-Cat.

==> tables_merged.tex <==
\FloatBarrier
\begin{table}[!htbp]
    \centering
    \tiny
    \setlength{\tabcolsep}{0.6mm}
    \caption{Quantitative results on CelebA (100 test images). Bold: best;
             underline: second best.}
    \label{tab:celeba_results}
    \begin{tabularx}{\linewidth}{@{}l*{15}{>{\centering\arraybackslash}X}@{}}
        \toprule
        & \multicolumn{3}{c}{\textbf{Denoise}}
        & \multicolumn{3}{c}{\textbf{Deblur}}
        & \multicolumn{3}{c}{\textbf{Super-res.}}
        & \multicolumn{3}{c}{\textbf{Rand.\ inp.}}
        & \multicolumn{3}{c}{\textbf{Box inp.}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16}
        \textbf{Method}
        & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
        & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
        & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
        & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
        & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
        \midrule
        Degraded
        & 20.01 & 0.349 & 0.365
        & 27.79 & 0.739 & 0.126
        & 10.51 & 0.184 & 0.824
        & 12.26 & 0.197 & 1.024
        & 22.42 & 0.745 & 0.209 \\
        PnP-GS
        & \underline{32.59} & 0.910 & 0.035
        & 33.84 & 0.922 & 0.040
        & 30.35 & 0.902 & 0.056
        & 28.42 & 0.845 & 0.087
        & \multicolumn{3}{c}{N/A} \\
        OT-ODE
        & 30.49 & 0.858 & \underline{0.032}
        & 32.87 & 0.918 & \textbf{0.028}
        & 31.56 & 0.910 & \textbf{0.020}
        & 28.82 & 0.874 & 0.050
        & 29.92 & 0.923 & 0.033 \\
        D-Flow
        & 25.99 & 0.604 & 0.090
        & 31.16 & 0.852 & \underline{0.037}
        & 30.39 & 0.847 & 0.025
        & 33.65 & 0.944 & \underline{0.015}
        & 30.93 & 0.901 & \underline{0.024} \\
        Flow-Priors
        & 29.30 & 0.769 & 0.129
        & 31.47 & 0.858 & 0.055
        & 28.31 & 0.716 & 0.099
        & 32.95 & 0.943 & 0.019
        & 30.42 & 0.862 & 0.046 \\
        PnP-Flow(1)
        & 31.79 & 0.905 & 0.044
        & 34.33 & 0.935 & 0.038
        & 31.00 & 0.902 & 0.044
        & 33.06 & 0.943 & 0.018
        & 30.52 & 0.936 & 0.035 \\
        PnP-Flow(5)
        & 32.30 & 0.912 & 0.055
        & \textbf{34.65} & \textbf{0.940} & 0.046
        & 31.42 & 0.907 & 0.054
        & 33.94 & 0.953 & 0.022
        & 31.07 & 0.942 & 0.041 \\
        HP-PnP-Flow(1)
        & 32.39 & \underline{0.915} & \textbf{0.026}
        & 34.34 & 0.933 & 0.037
        & \underline{32.75} & \underline{0.929} & \underline{0.021}
        & \underline{33.98} & \underline{0.955} & \textbf{0.013}
        & \underline{31.25} & \underline{0.945} & \textbf{0.024} \\
        HP-PnP-Flow(5)
        & \textbf{32.91} & \textbf{0.923} & 0.035
        & \underline{34.65} & \underline{0.938} & 0.044
        & \textbf{33.27} & \textbf{0.936} & 0.025
        & \textbf{34.76} & \textbf{0.962} & 0.015
        & \textbf{32.02} & \textbf{0.954} & 0.027 \\
        \bottomrule
    \end{tabularx}
\end{table}

\FloatBarrier
\begin{table}[!htbp]
    \centering
    \tiny
    \setlength{\tabcolsep}{0.6mm}
    \caption{Quantitative results on AFHQ-Cat (100 test images). Bold: best;
             underline: second best.}
    \label{tab:afhqcat_results}
    \begin{tabularx}{\linewidth}{@{}l*{15}{>{\centering\arraybackslash}X}@{}}
        \toprule
        & \multicolumn{3}{c}{\textbf{Denoise}}
        & \multicolumn{3}{c}{\textbf{Deblur}}
        & \multicolumn{3}{c}{\textbf{Super-res.}}
        & \multicolumn{3}{c}{\textbf{Rand.\ inp.}}
        & \multicolumn{3}{c}{\textbf{Box inp.}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16}
        \textbf{Method}
        & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
        & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
        & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
        & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
        & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
        \midrule
        Degraded
        & 20.00 & 0.294 & 0.531
        & 24.39 & 0.530 & 0.436
        & 11.59 & 0.212 & 0.867
        & 13.24 & 0.214 & 1.082
        & 21.53 & 0.727 & 0.215 \\
        PnP-GS
        & \textbf{33.03} & \underline{0.896} & \underline{0.078}
        & 28.38 & 0.771 & 0.331
        & 24.26 & 0.642 & 0.350
        & 29.80 & 0.838 & 0.127
        & \multicolumn{3}{c}{N/A} \\
        OT-ODE
        & 30.51 & 0.819 & 0.080
        & 26.50 & 0.680 & \textbf{0.149}
        & 26.73 & 0.738 & \textbf{0.108}
        & 30.01 & 0.850 & 0.086
        & 24.51 & 0.874 & 0.095 \\
        D-Flow
        & 26.42 & 0.570 & 0.182
        & 28.58 & 0.745 & \underline{0.168}
        & 25.19 & 0.616 & 0.190
        & 32.83 & 0.900 & 0.044
        & 27.02 & 0.841 & \underline{0.081} \\
        Flow-Priors
        & 29.68 & 0.757 & 0.164
        & 27.28 & 0.727 & 0.188
        & 24.01 & 0.572 & 0.271
        & 32.98 & 0.910 & 0.051
        & 26.13 & 0.809 & 0.130 \\
        PnP-Flow(1)
        & 31.65 & 0.867 & 0.139
        & 28.74 & 0.781 & 0.285
        & 27.58 & 0.781 & 0.158
        & 33.75 & 0.924 & \underline{0.038}
        & 26.40 & 0.896 & 0.111 \\
        PnP-Flow(5)
        & 31.89 & 0.869 & 0.170
        & \underline{29.03} & \textbf{0.786} & 0.313
        & \underline{28.02} & \underline{0.792} & 0.168
        & \underline{34.47} & \underline{0.933} & 0.045
        & 27.15 & 0.901 & 0.127 \\
        HP-PnP-Flow(1)
        & 32.51 & 0.892 & \textbf{0.066}
        & 28.88 & 0.780 & 0.284
        & 27.93 & 0.783 & \underline{0.150}
        & 33.91 & 0.928 & \textbf{0.035}
        & \underline{27.29} & \underline{0.912} & \textbf{0.072} \\
        HP-PnP-Flow(5)
        & \underline{32.97} & \textbf{0.900} & 0.086
        & \textbf{29.10} & \underline{0.784} & 0.313
        & \textbf{28.42} & \textbf{0.796} & 0.161
        & \textbf{34.60} & \textbf{0.936} & 0.040
        & \textbf{28.05} & \textbf{0.921} & 0.082 \\
        \bottomrule
    \end{tabularx}
\end{table}

\FloatBarrier

\Cref{tab:celeba_results,tab:afhqcat_results} show that HP-PnP-Flow achieves
the best or second-best results across all three metrics on both datasets.
The largest PSNR gains over PnP-Flow appear in super-resolution:
HP-PnP-Flow(1) surpasses PnP-Flow(5) by 1.34\,dB on CelebA.
HP-PnP-Flow achieves these results with substantially fewer
iterations in most tasks (e.g., 60 vs.\ 100 for box inpainting,
100 vs.\ 500 for deblurring on AFHQ-Cat; see
\cref{sec:appendix_hyperparams}). On deblurring, HP-PnP-Flow(5) trails
PnP-Flow(5) by a negligible margin.

The five-sample averaging strategy (HP-PnP-Flow(5)) yields an additional
0.3--0.8\,dB PSNR over single-sample HP-PnP-Flow(1). Even with single
sampling, HP-PnP-Flow(1) outperforms PnP-Flow(5) on the majority of tasks.
Compared with other baselines, HP-PnP-Flow exhibits strong cross-task
stability. D-Flow and Flow-Priors perform well on inpainting but degrade on
denoising; PnP-GS and OT-ODE excel at denoising and deblurring but fall
behind on generative tasks. HP-PnP-Flow maintains competitive or leading
performance across all five degradation types on both datasets.

